Dynamic-TreeRPO: Breaking the Independent Trajectory Bottleneck with Structured Sampling

The integration of Reinforcement Learning (RL) into flow matching models for text-to-image (T2I) generation has driven substantial advances in generation quality. However, these gains often come at the cost of exhaustive exploration and inefficient sampling strategies due to slight variation in the sampling group. Building on this insight, we propose Dynamic-TreeRPO, which implements the sliding-window sampling strategy as a tree-structured search with dynamic noise intensities along depth. We perform GRPO-guided optimization and constrained Stochastic Differential Equation (SDE) sampling within this tree structure. By sharing prefix paths of the tree, our design effectively amortizes the computational overhead of trajectory search. With well-designed noise intensities for each tree layer, Dynamic-TreeRPO can enhance the variation of exploration without any extra computational cost. Furthermore, we seamlessly integrate Supervised Fine-Tuning (SFT) and RL paradigm within Dynamic-TreeRPO to construct our proposed LayerTuning-RL, reformulating the loss function of SFT as a dynamically weighted Progress Reward Model (PRM) rather than a separate pretraining method. By associating this weighted PRM with dynamic-adaptive clipping bounds, the disruption of exploration process in Dynamic-TreeRPO is avoided. Benefiting from the tree-structured sampling and the LayerTuning-RL paradigm, our model dynamically explores a diverse search space along effective directions. Compared to existing baselines, our approach demonstrates significant superiority in terms of semantic consistency, visual fidelity, and human preference alignment on established benchmarks, including HPS-v2.1, PickScore, and ImageReward. In particular, our model outperforms SoTA by $4.9\%$, $5.91\%$, and $8.66\%$ on those benchmarks, respectively, while improving the training efficiency by nearly $50\%$.

==> Tables/ablation_main.tex <==
\begin{tabular}{{ccc|ccccccc}}
\midrule
{Dynamic-Tree} & {Dynamic-Clipping} & {LayerTuning-RL}& HPS-v2.1$\uparrow$  & Pick Score$\uparrow$  & ImageReward$\uparrow$   \\

\midrule
\xmark & \xmark & \xmark &  0.313 & 0.227 & 1.088  \\

\midrule
\cmark & \xmark & \xmark &  0.361\textcolor{blue}{(+0.048)} & 0.238\textcolor{blue}{(+0.011)} & 1.591\textcolor{blue}{(+0.503)}  \\

\midrule
\cmark & \cmark & \xmark &  0.369\textcolor{blue}{(+0.056)} & 0.242\textcolor{blue}{(+0.015)} & 1.674\textcolor{blue}{(+0.586)}  \\

\midrule
\cmark & \cmark & \cmark &  0.385\textcolor{blue}{(+0.072)} & 0.251\textcolor{blue}{(+0.024)} & 1.770\textcolor{blue}{(+0.682)}  \\
\midrule
\end{tabular}

% \begin{table}[t]
% \centering
% \caption{Ablation study of MixGRPO components. Each row adds one component on top of the previous setting. Metrics: higher is better ($\uparrow$).}
% \label{tab:ablation}
% \begin{tabular}{l S[table-format=1.3] S[table-format=1.3] S[table-format=1.3]}
% \toprule
% \textbf{Configuration} & \textbf{HPS-v2.1$\uparrow$} & \textbf{Pick Score$\uparrow$} & \textbf{ImageReward$\uparrow$} \\
% \midrule
% Baseline (none)               & 0.313 & 0.227 & 1.088 \\
% + Dynamic-Tree                & 0.361 & 0.238 & 1.591 \\
% + Dynamic-Clipping            & 0.369 & 0.242 & 1.674 \\
% + LayerTuning-RL              & 0.385 & 0.251 & 1.770 \\
% \bottomrule
% \end{tabular}
% \end{table}
